One-Shot Triple-Resource Trade-Off in Quantum Channel Coding

We analyze a task in which classical and quantum messages are simultaneously communicated via a noisy quantum channel, assisted with a limited amount of shared entanglement. We derive direct and converse bounds for the one-shot capacity region, represented by the smooth conditional entropies and the error tolerance. The proof is based on the randomized partial decoupling theorem, which is a generalization of the decoupling theorem. The two bounds match in the asymptotic limit of infinitely many uses of a memoryless channel and coincide with the previous result obtained by Hsieh and Wilde. Direct and converse bounds for various communication tasks are obtained as corollaries, both for the one-shot and asymptotic scenarios.

==> conclusion_1.tex <==
In this paper, we have analyzed the task of simultaneously transmitting classical and quantum messages through a noisy quantum channel, assisted by a limited amount of shared entanglement. 
We have considered a single-shot scenario and derived the direct and converse bounds for the achievable triplets of classical communication, quantum communication, and entanglement consumption.  
To our knowledge, this is the first time that the full trade-off relation among the three resources has been obtained in the one-shot channel coding scenario.
We have also applied the one-shot result to the asymptotic scenario of infinitely many uses of the identical channel. 
We have fully characterized the achievable rate region, which coincides with the prior result based on the resource inequality calculus \cite{hsieh2010entanglement}. 
Numerical calculations of the achievable rate region for specific qubit channels are given in \cite{nakata2021one}. In \cite{wakakuwa2020one}, we also analyze quantum state redistribution for a classical-quantum hybrid source in the one-shot scenario in terms of randomized partial decoupling. To investigate relations between these two tasks is left as future work.


Complementary to the decoupling-based approach is the one based on hypothesis testing (see Table I).
This approach has an advantage over the decoupling approach in that it recovers the optimal asymptotic results not only in the i.i.d. setting but also in the non-i.i.d. (information spectrum) setting when restricted to communication of classical messages.
In this approach, the concepts of convex splitting and position-based coding have recently proved useful in various settings of one-shot quantum channel coding \cite{qi2018applications,salek2019one,anshu2018building,anshu2019near,salek2018one,wilde2017position}.
However, most of these results only deal with communication of classical messages and do not cover quantum ones.
A possible reason is that the hypothesis-testing approach is based on the reduction of decoding classical messages to testing quantum hypothesis, which is not directly applicable to quantum communication.
Ref.~\cite{salek2019one} argues that this limitation can be removed by utilizing the equivalence between the quantum capacity and the private classical capacity of a quantum channel \cite{devetak2005private}.
Based on this argument, Ref.~\cite{salek2019one} considers the simultaneous transmission of classical and quantum messages without the assistance of entanglement.
But it is not clear whether this can be extended without sacrificing the asymptotic optimality to the case with limited entanglement assistance.
To our knowledge, the hypothesis testing approach has not succeeded in simultaneously dealing with all of the three resources of classical communication, quantum communication, and entanglement.
It is left as future work to obtain an asymptotically optimal one-shot three-dimensional rate region that incorporates all three resources.

==> conclusion_2.tex <==
In this paper, we have analyzed the task of simultaneously transmitting classical and quantum messages through a noisy quantum channel assisted by a limited amount of shared entanglement, all in the one-shot scenario. 
We have derived direct and converse bounds for the achievable triplets of classical communication, quantum communication, and entanglement consumption.  
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
We then applied the one-shot result to the asymptotic scenario of infinitely many uses of the identical channel.
We obtained a full characterization of the triple resource trade-offs, which coincides with the prior result based on the resource inequality calculus \cite{hsieh2010entanglement}. 
Numerical calculations of the achievable rate region for specific qubit channels are given in \cite{nakata2021one}. 
In \cite{wakakuwa2020one}, we also analyze quantum state redistribution for a classical-quantum hybrid source in the one-shot scenario in terms of randomized partial decoupling. 
To investigate relations between these two tasks is left as future work.



==> conclusion_3.tex <==
In this paper, we have analyzed the task of simultaneously transmitting classical and quantum messages through a noisy quantum channel assisted by a limited amount of shared entanglement, all in the one-shot scenario. 
We have derived direct and converse bounds for the achievable triplets of classical communication, quantum communication, and entanglement consumption.  
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
We then applied the one-shot result to the asymptotic scenario of infinitely many uses of the identical channel.
We obtained a full characterization of the triple resource trade-offs, which coincides with the prior result based on the resource inequality calculus \cite{hsieh2010entanglement}. 
Numerical calculations of the achievable rate region for specific qubit channels are given in \cite{nakata2021one}. 
In \cite{wakakuwa2020one}, we also analyze quantum state redistribution for a classical-quantum hybrid source in the one-shot scenario in terms of randomized partial decoupling. 
To investigate relations between these two tasks is left as future work.



Complementary to the decoupling-based approach is the one based on hypothesis testing \cite{mosonyi2009generalized,wang2012one,tomamichel2016quantum,matthews2014finite,datta2016second,salek2019one,}.
This approach has an advantage over the decoupling approach in that it recovers the optimal asymptotic results not only in the i.i.d. setting but also in the non-i.i.d. (information spectrum) setting when restricted to communication of classical messages.
In particular, the concepts of convex splitting and position-based coding have recently proved useful in various settings of one-shot quantum channel coding \cite{qi2018applications,salek2019one,anshu2018building,anshu2019near,salek2018one,wilde2017position,}.
However, none of them has succeeded in simultaneously dealing with all the three resources of classical communication, quantum communication and entanglement.
It is left as future work to obtain an asymptotically optimal one-shot three-dimensional rate region that incorporates all three resources.



==> conclusion_4.tex <==


In this paper, we have analyzed the task of simultaneously transmitting classical and quantum messages through a noisy quantum channel assisted by a limited amount of shared entanglement in the one-shot scenario. 
We have derived direct and converse bounds for the one-shot achievable rate region.  
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
We then applied the one-shot result to the asymptotic scenario of infinitely many uses of the identical channel.
We obtained a full characterization of the triple resource trade-offs, which coincides with the prior result by Hsieh and Wilde \cite{hsieh2010entanglement}. 
Numerical calculations of the achievable rate region for specific qubit channels are given in \cite{nakata2021one}. 
In \cite{wakakuwa2020one}, we analyzed quantum state redistribution for a classical-quantum hybrid source in the one-shot scenario in terms of randomized partial decoupling. 
To investigate relations between these two tasks is left as a future work.



{\red Complementary to the decoupling approach is the one based on hypothesis testing \cite{mosonyi2009generalized,wang2012one,tomamichel2016quantum,matthews2014finite,datta2016second,salek2019one,}.}
This approach has an advantage over the decoupling approach in that it recovers the optimal asymptotic results not only in the i.i.d. setting but also in the non-i.i.d. (information spectrum) setting.
{\red In particular, the concepts of convex splitting and position-based coding have recently proved useful in various settings of one-shot quantum channel coding \cite{qi2018applications,salek2019one,anshu2018building,anshu2019near,salek2018one,wilde2017position,}.}
It is left as future work to obtain an asymptotically optimal one-shot three-dimensional rate region that incorporates all three resources.



==> conclusion_5.tex <==


In this paper, we have analyzed the task of simultaneously transmitting classical and quantum messages through a noisy quantum channel assisted by a limited amount of shared entanglement in the one-shot scenario. 
We have derived direct and converse bounds for the one-shot achievable rate region.  
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
We then applied the one-shot result to the asymptotic scenario of infinitely many uses of the identical channel.
We obtained a full characterization of the triple resource trade-offs, which coincides with the prior result by Hsieh and Wilde \cite{hsieh2010entanglement}. 
Numerical calculations of the achievable rate region for specific qubit channels are given in \cite{nakata2021one}. 
In \cite{wakakuwa2020one}, we analyzed quantum state redistribution for a classical-quantum hybrid source in the one-shot scenario in terms of randomized partial decoupling. 
To investigate relations between these two tasks is left as a future work.



To quantum channel coding problems in the one-shot scenario, an approach from hypothesis testing (see e.g.~\cite{mosonyi2009generalized,wang2012one,tomamichel2016quantum,matthews2014finite,datta2013smooth,datta2016second,salek2019one,wilde2017converse}) is complementary to the one based on decoupling.
This approach has an advantage over the decoupling approach in that it recovers the optimal asymptotic results not only in the i.i.d. setting but also in the non-i.i.d. (information spectrum) setting.
The hypothesis-testing approach has been widely used for quantum channel coding problems to investigate e.g.~the strong converse exponent and the second-order asymptotics.
Along this line, the concepts of convex splitting \cite{anshu2017quantum} and position-based coding \cite{anshu2018building} have recently proved useful in various settings of one-shot quantum channel coding \cite{qi2018applications,salek2019one,anshu2018building,anshu2019near,salek2018one,wilde2017position,gagatsos2020covert,sen2021inner,wang2022towards,anshu2022efficient,salek2020single,salek2019publicness}.
One future direction is to apply the hypothesis-testing approach to the problem addressed in this paper and to obtain a triple-resource trade-off bounds that are asymptotically tight in the non-i.i.d. setting.



==> conclusion_6.tex <==


In this paper, we analyzed the task of simultaneously transmitting classical and quantum messages through a noisy quantum channel assisted by a limited amount of shared entanglement in the one-shot scenario. 
We have derived direct and converse bounds for the one-shot achievable rate region.  
To our knowledge, this is the first time that trade-off relations that apply simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
We then applied the one-shot result to the asymptotic scenario of infinitely many uses of a memoryless channel.
We obtained a complete characterization of the triple resource trade-offs, which coincides with the prior result by Hsieh and Wilde \cite{hsieh2010entanglement}. 
Numerical calculations of the achievable rate region for specific qubit channels are given in \cite{nakata2021one}. 
In \cite{wakakuwa2020one}, we analyzed quantum state redistribution for a classical-quantum hybrid source in the one-shot scenario in terms of randomized partial decoupling. 
To investigate relations between these two tasks is left as future work.



To investigate quantum channel coding problems in the one-shot scenario, an approach from hypothesis testing (see e.g.~\cite{mosonyi2009generalized,wang2012one,tomamichel2016quantum,matthews2014finite,datta2013smooth,datta2016second,salek2019one,wilde2017converse}) is complementary to the one based on decoupling.
The hypothesis-testing approach has an advantage over the decoupling approach in that it recovers the optimal asymptotic results not only in the i.i.d. setting but also in the non-i.i.d. (information spectrum) setting.
This approach has been widely used for quantum channel coding problems e.g.~to investigate the strong converse bounds and the second-order asymptotics.
Along this line, the concepts of convex splitting \cite{anshu2017quantum} and position-based coding \cite{anshu2018building} have recently proved useful in various settings of one-shot quantum channel coding \cite{qi2018applications,salek2019one,anshu2018building,anshu2019near,salek2018one,wilde2017position,gagatsos2020covert,sen2021inner,wang2022towards,anshu2022efficient,salek2020single,salek2019publicness}.
One future direction is to apply the hypothesis-testing approach to the problem addressed in this paper and obtain triple-resource trade-off bounds that are asymptotically tight in the non-i.i.d. setting.



==> introduction_1.tex <==
One of the major goals of quantum communication theory is to investigate the ultimate capacities of a noisy quantum channel for transmitting classical and quantum information, in particular those in an asymptotic limit of many uses of a discrete memoryless channel (see, e.g., \cite{wildetext,nielsentext}).
Classical and quantum capacities of a noisy quantum channel were obtained in \cite{holevo98,schumacher97,bennett1999entanglement} and \cite{lloyd1997capacity,devetak2005private,devetak2004family}, respectively, for entanglement non-assisted and assisted scenarios.
The capacity of a quantum channel for simultaneously transmitting classical and quantum messages was obtained in \cite{devetak2005capacity,hsieh2010entanglement}.
Refs.~\cite{devetak2004relating,devetak2005distillation} provided a unified approach to another goal of quantum communication theory, namely, evaluation of the maximum amount of pure entanglement or secrecy that one can extract from a mixed quantum state. 
Subsequently, this result was developed into quantum state merging \cite{horo05,horo07}, the fully quantum Slepian-Wolf (FQSW) protocol \cite{ADHW2009}, and state redistribution \cite{devetak2008exact,yard2009optimal}.
Remarkably, various coding theorems, including quantum capacity theorems, are obtained by reduction from FQSW \cite{ADHW2009}.
These results lead to a unified view for various quantum communication tasks, referred to as the protocol family \cite{ADHW2009,devetak2004family}.




The concept of decoupling plays a central role in the above analyses of quantum protocols. Decoupling refers to destroying the correlation between two quantum systems by applying an operation on one of the two subsystems. In various scenarios, the amount of communication required for accomplishing a quantum protocol equals the amount of ``randomness'' of the operation that decouples a particular quantum state (see, e.g., \cite{horo07,ADHW2009}). The decoupling approach simplifies many problems of our interest because any purification of a mixed quantum state is convertible to another reversibly.
This fact, known as Uhlmann's theorem \cite{uhlmann1976transition}, enables us to prove the existence of a suitable decoder for quantum communication without explicitly constructing it.





The decoupling approach to quantum protocols has been generalized to the one-shot scenario.
Ref.~\cite{DBWR2010} proved one of the most general formulations of decoupling, which is referred to as the {\it one-shot decoupling theorem}.
The decoupling theorem provides a necessary condition and a sufficient condition for an operation to decouple a quantum state with high precision.
The conditions are represented in terms of smooth min- and max- entropies of the operation and the state.
Various coding theorems in the one-shot scenario are obtained from the decoupling theorem~\cite{fred10_2} in the same way as in the asymptotic scenario.
Furthermore, due to the fully quantum asymptotic equipartition property \cite{tomamichel2009fully}, the results also reconstruct the previous results in the asymptotic scenario.
A generalization and refinement of the decoupling theorem, called {\it catalytic decoupling}, was also proposed in \cite{majenz2017catalytic}.



There is, however, a limitation in the decoupling approach in that it does not incorporate classical communication tasks. 
Classical communication over noisy quantum channels was addressed in Ref.~\cite{dupuis2014decoupling} using a decoupling-like approach based on the {\it dequantizing theorem}. However, it still does not fully incorporate a general scenario in which classical and quantum messages are simultaneously transmitted, possibly with the assistance of shared entanglement. 
To address this scenario by the existing decoupling methods, we need to apply the decoupling theorem and the dequantizing theorem separately for the two sources (see also Refs.~\cite{salek2019one} for a different approach based on the convex splitting).
From this viewpoint, the unified approach to communication over noisy quantum channels based on decoupling has not been fully completed.



\begin{table*}[t]
\renewcommand{\arraystretch}{1.5}
  \begin{center}
    \begin{tabular}{c|c|c|c|c|c} \hline
	 & \multicolumn{2}{c}{decoupling}                  &  \multicolumn{2}{|c|}{hypothesis testing} & other \\\cline{2-6}
            &   direct &  converse  &  direct &  converse  & direct/converse \\ \hline
    \multirow{2}{*}{$c$}   &    \multirow{2}{*}{Dupuis et al.~\cite{dupuis2014decoupling}} &         \multirow{2}{*}{-}                                  & \multicolumn{2}{c|}{ \begin{tabular}{c} Mosonyi et al.~\cite{mosonyi2009generalized}, Wang et al.~\cite{wang2012one}, \\[-1mm] Datta et al.~\cite{datta2013smooth}  \end{tabular} } &  \multirow{2}{*}{Renes et al.~\cite{renes2011noisy}} \\\cline{4-5}
    	& 	&	&	-	&  Matthews et al.~\cite{matthews2014finite}	&    \\\hline
   $q$ &   \multicolumn{2}{|c|}{Datta et al.~\cite{datta2011apex}, Buscemi et al.~\cite{buscemi2010quantum}}                         & - & -	&- \\\hline
   $c$, $q$ &  -  &                    -             & \multicolumn{2}{|c|}{Salek et al.~\cite{salek2019one}} & - \\ \hline
   \multirow{2}{*}{\begin{tabular}{c}\white{-} \\ \; $c$, $e$ \end{tabular} } & \multicolumn{2}{|c|}{}     &  \multicolumn{2}{|c|}{Qi et al.~\cite{qi2018applications}} &	\multirow{3}{*}{-}\\ \cline{4-5}
     & \multicolumn{2}{|c|}{ \begin{tabular}{c} Datta et al.~\cite{datta2012one}   \\  \white{-} \end{tabular}        }     &  \begin{tabular}{c} Datta et al.~\cite{datta2016second}, \\[-1mm] Anshu et al.~\cite{anshu2018building}  \end{tabular}  & \begin{tabular}{c} Matthews et al.~\cite{matthews2014finite}, \\[-1mm] Anshu et al.~\cite{anshu2019near}  \end{tabular} &	\\ \hline
   $q$, $e$ & \multicolumn{2}{|c|}{Datta et al.~\cite{datta2012one}         }        & - & -	&	-\\\hline
   $c$, $q$, $e$ & \multicolumn{2}{|c|}{[THIS PAPER]}       & - & -	&-	\\\hline
   \multirow{2}{*}{private} &  \multirow{2}{*}{-} & \multirow{2}{*}{-}  & \multicolumn{2}{|c|}{Salek et al. \cite{salek2018one}} 	&	\multirow{2}{*}{ \begin{tabular}{c} Renes et al.~\cite{renes2011noisy},   \\[-1mm]  Radhakrishnan et al.~\cite{radhakrishnan2017one}, \end{tabular}      } \\\cline{4-5}
       & & & Wilde ~\cite{wilde2017position} & -	& \\\hline
    \end{tabular}
  \end{center}
  \caption{ Prior works on the one-shot capacities of a quantum channel.
}
  \label{tb:values}
\end{table*}




This paper proposes a unified decoupling approach that allows us to simultaneously treat classical communication, quantum communication, and shared entanglement.
Namely, we consider a task in which classical and quantum messages are transmitted via a noisy quantum channel with the assistance of a limited amount of shared entanglement. 
This task was analyzed in \cite{hsieh2010entanglement} for an asymptotic scenario, whereas we consider the one-shot scenario based on the decoupling approach. 
The main result is that we derive a one-shot rate region for this task, which is represented in terms of the smooth conditional entropy of the channel.
To our knowledge, this is the first time that the whole trade-off relation among the resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
The direct and converse bounds for various communication tasks in the one-shot scenario readily follow from this result.
In the asymptotic limit of infinitely many uses of the channel, the direct and converse bounds coincide and recover the entire achievable rate region obtained in \cite{hsieh2010entanglement}.



The proof is based on the {\it randomized partial decoupling} \cite{wakakuwa2021one}, which is a generalization of decoupling.
Here, we consider a scenario in which a bipartite quantum state on system $AR$ is subject to a unitary operation on $A$, followed by the action of a linear completely-positive (CP) map. Unlike the usual setting of decoupling, we assume that
the subsystem is decomposed into a direct-sum form, and 
the unitary is chosen at random from the set of unitaries that are block-diagonal under the decomposition. 
In \cite{wakakuwa2021one}, we proved the {\it randomized partial decoupling theorem}, which shows that the distance between the final state and the averagesd one is bounded in terms of smooth conditional entropies of the initial state and the channel.
The previous results of the one-shot decoupling theorem \cite{DBWR2010} and the dequantization theorem \cite{dupuis2014decoupling}
are obtained from this result as corollaries (see Section III D in \cite{wakakuwa2021one} for the details).



We summarize prior works on the one-shot capacity of quantum channels in various scenarios in Table \ref{tb:values}. Most of them are classified into approaches based on decoupling and quantum hypothesis testing. The tasks analyzed therein are mostly communication of classical message ($c$) or quantum message ($q$) or both $(c,q)$, with or without the assistance of shared entanglement ($e$). 
The result presented in this paper incorporates all these scenarios as special cases. 
We leave it for future work to see whether our result applies to the task of privately communicating classical messages.
We expect that this can be done by exploiting the equivalence between quantum communication and private classical communication over a noisy quantum channel, which was first introduced in \cite{devetak2005private} for the asymptotic scenario and was applied in \cite{salek2019one} to the one-shot scenario.


This paper is organized as follows. 
In \rSec{prelimi}, we introduce notations and definitions that will be used throughout this paper. 
In \rSec{RPD}, we summarize the statement of the randomized partial decoupling theorem.
In \rSec{mainresults}, we present formulations of the problem and the main results. 
The proofs of the main theorems are provided in Section \rsec{direct} and \rsec{converse}.


==> introduction_2.tex <==
%One of the major goals of quantum communication theory is to investigate the ultimate capacities of a noisy quantum channel for transmitting classical and quantum information, in particular those in an asymptotic limit of many uses of a discrete memoryless channel (see, e.g., \cite{wildetext,nielsentext}).
%Classical and quantum capacities of a noisy quantum channel were obtained in \cite{holevo98,schumacher97,bennett1999entanglement} and \cite{lloyd1997capacity,devetak2005private,devetak2004family}, respectively, for entanglement non-assisted and assisted scenarios.
%The capacity of a quantum channel for simultaneously transmitting classical and quantum messages was obtained in \cite{devetak2005capacity,hsieh2010entanglement}.
%Refs.~\cite{devetak2004relating,devetak2005distillation} provided a unified approach to another goal of quantum communication theory, namely, evaluation of the maximum amount of pure entanglement or secrecy that one can extract from a mixed quantum state. 
%Subsequently, this result was developed into quantum state merging \cite{horo05,horo07}, the fully quantum Slepian-Wolf (FQSW) protocol \cite{ADHW2009}, and state redistribution \cite{devetak2008exact,yard2009optimal}.
%Remarkably, various coding theorems, including quantum capacity theorems, are obtained by reduction from FQSW \cite{ADHW2009}.
%These results lead to a unified view for various quantum communication tasks, referred to as the protocol family \cite{ADHW2009,devetak2004family}.
%
%
%
%
%The concept of decoupling plays a central role in the above analyses of quantum protocols. Decoupling refers to destroying the correlation between two quantum systems by applying an operation on one of the two subsystems. In various scenarios, the amount of communication required for accomplishing a quantum protocol equals the amount of ``randomness'' of the operation that decouples a particular quantum state (see, e.g., \cite{horo07,ADHW2009}). The decoupling approach simplifies many problems of our interest because any purification of a mixed quantum state is convertible to another reversibly.
%This fact, known as Uhlmann's theorem \cite{uhlmann1976transition}, enables us to prove the existence of a suitable decoder for quantum communication without explicitly constructing it.
%
%
%
%
%
%The decoupling approach to quantum protocols has been generalized to the one-shot scenario.
%Ref.~\cite{DBWR2010} proved one of the most general formulations of decoupling, which is referred to as the {\it one-shot decoupling theorem}.
%The decoupling theorem provides a necessary condition and a sufficient condition for an operation to decouple a quantum state with high precision.
%The conditions are represented in terms of smooth min- and max- entropies of the operation and the state.
%Various coding theorems in the one-shot scenario are obtained from the decoupling theorem~\cite{fred10_2} in the same way as in the asymptotic scenario.
%Furthermore, due to the fully quantum asymptotic equipartition property \cite{tomamichel2009fully}, the results also reconstruct the previous results in the asymptotic scenario.
%A generalization and refinement of the decoupling theorem, called {\it catalytic decoupling}, was also proposed in \cite{majenz2017catalytic}.
%
%
%

%
%
%
%\begin{table*}[t]
%\renewcommand{\arraystretch}{1.5}
%  \begin{center}
%    \begin{tabular}{c|c|c|c|c|c} \hline
%	 & \multicolumn{2}{c}{decoupling}                  &  \multicolumn{2}{|c|}{hypothesis testing} & other \\\cline{2-6}
%            &   direct &  converse  &  direct &  converse  & direct/converse \\ \hline
%    \multirow{2}{*}{$c$}   &    \multirow{2}{*}{Dupuis et al.~\cite{dupuis2014decoupling}} &         \multirow{2}{*}{-}                                  & \multicolumn{2}{c|}{ \begin{tabular}{c} Mosonyi et al.~\cite{mosonyi2009generalized}, Wang et al.~\cite{wang2012one}, \\[-1mm] Datta et al.~\cite{datta2013smooth}  \end{tabular} } &  \multirow{2}{*}{Renes et al.~\cite{renes2011noisy}} \\\cline{4-5}
%    	& 	&	&	-	&  Matthews et al.~\cite{matthews2014finite}	&    \\\hline
%   $q$ &   \multicolumn{2}{|c|}{Datta et al.~\cite{datta2011apex}, Buscemi et al.~\cite{buscemi2010quantum}}                         & - & -	&- \\\hline
%   $c$, $q$ &  -  &                    -             & \multicolumn{2}{|c|}{Salek et al.~\cite{salek2019one}} & - \\ \hline
%   \multirow{2}{*}{\begin{tabular}{c}\white{-} \\ \; $c$, $e$ \end{tabular} } & \multicolumn{2}{|c|}{}     &  \multicolumn{2}{|c|}{Qi et al.~\cite{qi2018applications}} &	\multirow{3}{*}{-}\\ \cline{4-5}
%     & \multicolumn{2}{|c|}{ \begin{tabular}{c} Datta et al.~\cite{datta2012one}   \\  \white{-} \end{tabular}        }     &  \begin{tabular}{c} Datta et al.~\cite{datta2016second}, \\[-1mm] Anshu et al.~\cite{anshu2018building}  \end{tabular}  & \begin{tabular}{c} Matthews et al.~\cite{matthews2014finite}, \\[-1mm] Anshu et al.~\cite{anshu2019near}  \end{tabular} &	\\ \hline
%   $q$, $e$ & \multicolumn{2}{|c|}{Datta et al.~\cite{datta2012one}         }        & - & -	&	-\\\hline
%   $c$, $q$, $e$ & \multicolumn{2}{|c|}{[THIS PAPER]}       & - & -	&-	\\\hline
%   \multirow{2}{*}{private} &  \multirow{2}{*}{-} & \multirow{2}{*}{-}  & \multicolumn{2}{|c|}{Salek et al. \cite{salek2018one}} 	&	\multirow{2}{*}{ \begin{tabular}{c} Renes et al.~\cite{renes2011noisy},   \\[-1mm]  Radhakrishnan et al.~\cite{radhakrishnan2017one}, \end{tabular}      } \\\cline{4-5}
%       & & & Wilde ~\cite{wilde2017position} & -	& \\\hline
%    \end{tabular}
%  \end{center}
%  \caption{ Prior works on the one-shot capacities of a quantum channel.
%}
%  \label{tb:values}
%\end{table*}


%
%
%
%
%We summarize prior works on the one-shot capacity of quantum channels in various scenarios in Table \ref{tb:values}. Most of them are classified into approaches based on decoupling and quantum hypothesis testing. The tasks analyzed therein are mostly communication of classical message ($c$) or quantum message ($q$) or both $(c,q)$, with or without the assistance of shared entanglement ($e$). 
%The result presented in this paper incorporates all these scenarios as special cases. 
%We leave it for future work to see whether our result applies to the task of privately communicating classical messages.
%We expect that this can be done by exploiting the equivalence between quantum communication and private classical communication over a noisy quantum channel, which was first introduced in \cite{devetak2005private} for the asymptotic scenario and was applied in \cite{salek2019one} to the one-shot scenario.

One of the most general result in this direction is provided in \cite{hsieh2010entanglement}, which obtained the triple trade-off among the resources of classical communication, and quantum communication and entanglement in quantum channel coding.

However, in reality, the assumption of the asymptotic limit of infinitely many uses of a channel is too idealized.
To overcome this limitation, the one-shot approach has been developed.
Among various scenarios, the classical capacity of a quantum channel is investigated in \cite{dupuis2014decoupling,mosonyi2009generalized,wang2012one,datta2013smooth,renes2011noisy,matthews2014finite,}, the quantum capacity in \cite{datta2011apex,buscemi2010quantum,}, the entanglement-assisted classical and quantum capacities are analyzed in \cite{qi2018applications,datta2012one,datta2016second,anshu2018building,matthews2014finite,anshu2019near,} and \cite{datta2012one,}, respectively, the simultaneous transmission of classical and quantum information is investigated in \cite{salek2019one,}, and the private classical capacity is analyzed in \cite{salek2018one,renes2011noisy,radhakrishnan2017one,wilde2017position,}.
However, the one-shot capacity theorem that reduces to the asymptotic result by Hsieh and Wilde has not been obtained so far.


This paper aims at generalizing the result by Hsieh and Wilde \cite{hsieh2010entanglement} to the one-shot scenario.
Namely, we consider a task in which classical and quantum messages are transmitted via a noisy quantum channel with the assistance of a limited amount of shared entanglement. 
This task was analyzed in \cite{hsieh2010entanglement} for an asymptotic scenario, whereas we consider the one-shot scenario based on the decoupling approach. 
The main result is that we derive a one-shot rate region for this task, which is represented in terms of the smooth conditional entropy of the channel.
To our knowledge, this is the first time that the whole trade-off relation among the resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
The direct and converse bounds for various communication tasks in the one-shot scenario readily follow from this result.
In the asymptotic limit of infinitely many uses of the channel, the direct and converse bounds coincide and recover the entire achievable rate region obtained in \cite{hsieh2010entanglement}.
It should be noted, however, that in special cases our result is not necessarily as strong as those in the previous literature.
To compare our result in detail with those in the previous literature is left as a future work.


The proof is based on the {\it randomized partial decoupling} \cite{wakakuwa2021one}, which is a generalization of decoupling.
Here, we consider a scenario in which a bipartite quantum state on system $AR$ is subject to a unitary operation on $A$, followed by the action of a linear completely-positive (CP) map. Unlike the usual setting of decoupling, we assume that
the subsystem is decomposed into a direct-sum form, and 
the unitary is chosen at random from the set of unitaries that are block-diagonal under the decomposition. 
In \cite{wakakuwa2021one}, we proved the {\it randomized partial decoupling theorem}, which shows that the distance between the final state and the averagesd one is bounded in terms of smooth conditional entropies of the initial state and the channel.
The previous results of the one-shot decoupling theorem \cite{DBWR2010} and the dequantization theorem \cite{dupuis2014decoupling}
are obtained from this result as corollaries (see Section III D in \cite{wakakuwa2021one} for the details).


This paper is organized as follows. 
In \rSec{prelimi}, we introduce notations and definitions that will be used throughout this paper. 
In \rSec{mainresults}, we present formulations of the problem and the main results. 
In \rSec{RPD}, we summarize the statement of the randomized partial decoupling theorem.
The proofs of the main theorems are provided in Section \rsec{direct} and \rsec{converse}.


==> introduction_3.tex <==




One of the major goals of quantum communication theory is to investigate the ultimate capacities of a noisy quantum channel for transmitting classical and quantum information, in particular those in an asymptotic limit of many uses of a discrete memoryless channel (see, e.g., \cite{wildetext,nielsentext}).
The classical capacity of a noisy quantum channel was obtained by Holevo \cite{holevo98}, Schumacher and Westmoreland  \cite{schumacher97}, and the quantum capacity was obtained by Lloyd \cite{lloyd1997capacity}, Shor \cite{shor2002quantum} and Devetak \cite{devetak2005private}.
The entanglement-assisted classical capacity was obtained by Bennet {\it et al.} \cite{bennett1999entanglement,bennett2002entanglement} and Shor \cite{shor2004classical}, and the entanglement-assisted quantum capacity was obtained by Devetak {\it et al.} \cite{devetak2004family,deve08}.
The capacity of a quantum channel for simultaneously transmitting classical and quantum messages was obtained in \cite{devetak2005capacity}.
One of the most general result in this direction is provided by Hsieh and Wilde \cite{hsieh2010entanglement}, which obtained the triple trade-off among the resources of classical communication, and quantum communication and entanglement in quantum channel coding.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases mentioned above are obtained from their result as corollaries.


However, in reality, the assumption of the asymptotic limit of infinitely many uses of a channel is too idealized.
To overcome this limitation, the one-shot approach has been developed.
The one-shot classical capacity of a noisy quantum channel was first investigated by Mosonyi {\it et al.} \cite{mosonyi2009generalized} and was developed by Renes {\it et al.} \cite{renes2011noisy} and Wang {\it et al.} \cite{wang2012one}.
The quantum capacity was obtained by Buscemi {\it et al.}\cite{buscemi2010quantum}.
The entanglement-assisted classical and quantum capacities were obtained by Datta {\it et al.} \cite{datta2012one}.
The one-shot capacity region for simultaneously transmitting classical and quantum information was obtained by Salek {\it et al.} \cite{salek2019one}.
In the asymptotic limit of infinitely many uses of a channel, all these results (except \cite{mosonyi2009generalized}) are known to coincide with their counterpart presented above.
Numerous studies have been done to further develop these approaches (see e.g.~\cite{dupuis2014decoupling,datta2013smooth,matthews2014finite,datta2011apex,qi2018applications,datta2016second,anshu2018building,anshu2019near}.)
However, the one-shot capacity theorem that reduces to the asymptotic result by Hsieh and Wilde has not been obtained so far.

%and the private classical capacity is analyzed in \cite{salek2018one,renes2011noisy,radhakrishnan2017one,wilde2017position,}.

In this paper, we derive a one-shot generalization of the three-dimensional rate region obtained in \cite{hsieh2010entanglement}. 
Namely, we consider a task in which classical and quantum messages are transmitted via a noisy quantum channel with the assistance of a limited amount of shared entanglement, all in the one-shot scenario. 
The main result is that we derive inner and outer bonds for a one-shot rate region for this task, which are represented in terms of the smooth conditional entropy of the channel.
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
In the asymptotic limit of infinitely many uses of the channel, the direct and converse bounds coincide and recover the entire achievable rate region obtained in \cite{hsieh2010entanglement}.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases such as $q=0,e=\infty$ are obtained from their result as corollaries.
Hence, our one-shot result result also recovers the capacity theorems in the asymptotic limit in those special cases.
Besides, the direct and converse bounds for various communication tasks in the one-shot scenario readily follow from this result.
It should be noted, however, that in special cases our result is not necessarily as strong as those in the previous literature.
To compare our result in detail with those in the previous literature is left as a future work.


The proof is based on the {\it randomized partial decoupling} \cite{wakakuwa2021one}, which is a generalization of decoupling.
Here, we consider a scenario in which a bipartite quantum state on system $AR$ is subject to a unitary operation on $A$, followed by the action of a linear completely-positive (CP) map. Unlike the usual setting of decoupling, we assume that
the subsystem is decomposed into a direct-sum form, and 
the unitary is chosen at random from the set of unitaries that are block-diagonal under the decomposition. 
In \cite{wakakuwa2021one}, we proved the {\it randomized partial decoupling theorem}, which shows that the distance between the final state and the averagesd one is bounded in terms of smooth conditional entropies of the initial state and the channel.
The previous results of the one-shot decoupling theorem \cite{DBWR2010} and the dequantization theorem \cite{dupuis2014decoupling}
are obtained from this result as corollaries (see Section III D in \cite{wakakuwa2021one} for the details).


Complementary to the decoupling-based approach is the one based on hypothesis testing.
This approach has an advantage over the decoupling approach in that it recovers the optimal asymptotic results not only in the i.i.d. setting but also in the non-i.i.d. (information spectrum) setting when restricted to communication of classical messages.
Along this line, the one-shot classical capacity of a noisy quantum channel was investigated by Mosonyi {\it et al.} \cite{mosonyi2009generalized} and Wang {\it et al.} \cite{wang2012one}.
The quantum capacity was obtained by Tomamichel {\it et al.} \cite{tomamichel2016quantum}.
The entanglement-assisted classical capacity was investigated by Matthews {\it et al.} \cite{matthews2014finite} and Datta {\it et al.} \cite{datta2016second}.
The result in \cite{datta2016second} also applies to the entanglement-assisted quantum capacity because of quantum teleportation \cite{bennett1993teleporting} and superdense coding \cite{bennett1992communication}.
The one-shot capacity region for simultaneously transmitting classical and quantum information was obtained by Salek {\it et al.} \cite{salek2019one}.
In the asymptotic limit of infinitely many uses of a channel, all these results (except \cite{mosonyi2009generalized}) are known to coincide with their counterpart presented above.
Numerous studies have been done to further develop these approaches (see e.g.~\cite{a}.)
In particular, the concepts of convex splitting and position-based coding have recently proved useful in various settings of one-shot quantum channel coding \cite{qi2018applications,salek2019one,anshu2018building,anshu2019near,salek2018one,wilde2017position}.
It is left as future work to obtain an asymptotically optimal one-shot three-dimensional rate region that incorporates all three resources.


This paper is organized as follows. 
In \rSec{prelimi}, we introduce notations and definitions that will be used throughout this paper. 
In \rSec{mainresults}, we present formulations of the problem and the main results. 
In \rSec{RPD}, we summarize the statement of the randomized partial decoupling theorem.
The proofs of the main theorems are provided in Section \rsec{direct} and \rsec{converse}.
In \rSec{iid}, we show that the one-shot inner and outer bounds coincide in the asymptotic limit of infinitely many uses of the channel, and recovers the three-dimensional capacity region obtained by Hsieh and Wilde \cite{}.
A detailed proof of this fact will be provided in \rApp{AEiid}.
Conclusions are presented in \rSec{cncl}.




==> introduction_4.tex <==




One of the major goals of quantum communication theory is to investigate the ultimate capacities of a noisy quantum channel for transmitting classical and quantum information, in particular those in an asymptotic limit of many uses of a discrete memoryless channel (see, e.g., \cite{wildetext,nielsentext}).
The classical capacity of a noisy quantum channel was obtained by Holevo \cite{holevo98}, Schumacher and Westmoreland  \cite{schumacher97}, and the quantum capacity was obtained by Lloyd \cite{lloyd1997capacity}, Shor \cite{shor2002quantum} and Devetak \cite{devetak2005private}.
The entanglement-assisted classical capacity was obtained by Bennet {\it et al.} \cite{bennett1999entanglement,bennett2002entanglement} and Shor \cite{shor2004classical}, and the entanglement-assisted quantum capacity was obtained by Devetak {\it et al.} \cite{devetak2004family,deve08}.
The capacity of a quantum channel for simultaneously transmitting classical and quantum messages was obtained in \cite{devetak2005capacity}.
One of the most general result in this direction is provided by Hsieh and Wilde \cite{hsieh2010entanglement}, which obtained the triple trade-off among the resources of classical communication, and quantum communication and entanglement in quantum channel coding.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases mentioned above are obtained from their result as corollaries.


However, in reality, the assumption of the asymptotic limit of infinitely many uses of a channel is too idealized.
To overcome this limitation, the one-shot approach has been developed.
The one-shot classical capacity of a noisy quantum channel was first investigated by Mosonyi {\it et al.} \cite{mosonyi2009generalized} and was developed by Renes {\it et al.} \cite{renes2011noisy} and Wang {\it et al.} \cite{wang2012one}.
The quantum capacity was obtained by Buscemi {\it et al.}\cite{buscemi2010quantum}.
The entanglement-assisted classical and quantum capacities were obtained by Datta {\it et al.} \cite{datta2012one}.
The one-shot capacity region for simultaneously transmitting classical and quantum information was obtained by Salek {\it et al.} \cite{salek2019one}.
In the asymptotic limit of infinitely many uses of a channel, all these results (except \cite{mosonyi2009generalized}) are known to coincide with their counterpart presented above.
Numerous studies have been done to further develop these approaches (see e.g.~\cite{dupuis2014decoupling,datta2013smooth,matthews2014finite,datta2011apex,qi2018applications,datta2016second,anshu2018building,anshu2019near}.)
However, the one-shot capacity theorem that reduces to the asymptotic result by Hsieh and Wilde has not been obtained so far.

%and the private classical capacity is analyzed in \cite{salek2018one,renes2011noisy,radhakrishnan2017one,wilde2017position,}.

In this paper, we derive a one-shot generalization of the three-dimensional rate region obtained in \cite{hsieh2010entanglement}. 
Namely, we consider a task in which classical and quantum messages are transmitted via a noisy quantum channel with the assistance of a limited amount of shared entanglement, all in the one-shot scenario. 
The main result is that we derive inner and outer bonds for a one-shot rate region for this task, which are represented in terms of the smooth conditional entropy of the channel.
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
In the asymptotic limit of infinitely many uses of the channel, the direct and converse bounds coincide and recover the entire achievable rate region obtained in \cite{hsieh2010entanglement}.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases such as $q=0,e=\infty$ are obtained from their result as corollaries.
Hence, our one-shot result result also recovers the capacity theorems in the asymptotic limit in those special cases.
Besides, the direct and converse bounds for various communication tasks in the one-shot scenario readily follow from this result.
It should be noted, however, that in special cases our result is not necessarily as strong as those in the previous literature.
To compare our result in detail with those in the previous literature is left as a future work.


The proof is based on the {\it randomized partial decoupling} \cite{wakakuwa2021one}, which is a generalization of decoupling.
Here, we consider a scenario in which a bipartite quantum state on system $AR$ is subject to a unitary operation on $A$, followed by the action of a linear completely-positive (CP) map. Unlike the usual setting of decoupling, we assume that
the subsystem is decomposed into a direct-sum form, and 
the unitary is chosen at random from the set of unitaries that are block-diagonal under the decomposition. 
In \cite{wakakuwa2021one}, we proved the {\it randomized partial decoupling theorem}, which shows that the distance between the final state and the averagesd one is bounded in terms of smooth conditional entropies of the initial state and the channel.
The previous results of the one-shot decoupling theorem \cite{DBWR2010} and the dequantization theorem \cite{dupuis2014decoupling}
are obtained from this result as corollaries (see Section III D in \cite{wakakuwa2021one} for the details).



This paper is organized as follows. 
In \rSec{prelimi}, we introduce notations and definitions that will be used throughout this paper. 
In \rSec{mainresults}, we present formulations of the problem and the main results. 
In \rSec{RPD}, we summarize the statement of the randomized partial decoupling theorem.
The proofs of the main theorems are provided in Section \rsec{direct} and \rsec{converse}.
In \rSec{iid}, we apply the one-shot results to the asymptotic limit of infinitely many uses of the channel, and obtain a three-dimensional achievable rate region region that is equivalent to the one obtained by Hsieh and Wilde.
A proof of the asymptotic result is provided in \rSec{PRFasymptotic}.
In \rSec{comparison}, we apply our results to special cases where one or only one or two resources are considered, and compare the results to those in the previous literature.
Conclusions are presented in \rSec{cncl}.




==> introduction_5.tex <==




One of the major goals of quantum communication theory is to investigate the ultimate capacities of a noisy quantum channel for transmitting classical and quantum information, in particular those in an asymptotic limit of many uses of a discrete memoryless channel (see, e.g., \cite{wildetext,nielsentext}).
The classical capacity of a noisy quantum channel was obtained by Holevo \cite{holevo98}, Schumacher and Westmoreland  \cite{schumacher97}.
The quantum capacity was obtained by Lloyd \cite{lloyd1997capacity}, Shor \cite{shor2002quantum} and Devetak \cite{devetak2005private}.
The entanglement-assisted classical capacity was obtained by Bennet {\it et al.} \cite{bennett1999entanglement,bennett2002entanglement} and Shor \cite{shor2004classical}, and the entanglement-assisted quantum capacity was obtained by Devetak {\it et al.} \cite{devetak2004family,deve08}.
The capacity of a quantum channel for simultaneously transmitting classical and quantum messages was obtained by Devetak and Shor \cite{devetak2005capacity}.
One of the most general result in this direction is provided by Hsieh and Wilde \cite{hsieh2010entanglement}, which obtained the triple trade-off among the resources of classical communication, and quantum communication and entanglement in quantum channel coding.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases mentioned above are obtained from their result as corollaries.


{\blue However, in reality, the assumption of the asymptotic limit of infinitely many uses of a channel is too idealized.
To overcome this limitation, the one-shot approach has been developed.}
The one-shot classical capacity of a noisy quantum channel was first investigated by Mosonyi {\it et al.} \cite{mosonyi2009generalized} and was developed by Renes {\it et al.} \cite{renes2011noisy} and Wang {\it et al.} \cite{wang2012one}.
The quantum capacity was obtained by Buscemi {\it et al.}\cite{buscemi2010quantum}.
The entanglement-assisted classical and quantum capacities were obtained by Datta {\it et al.} \cite{datta2012one}.
The one-shot capacity region for simultaneously transmitting classical and quantum information was obtained by Salek {\it et al.} \cite{salek2019one}.
In the asymptotic limit of infinitely many uses of a memoryless channel, all these results (except \cite{mosonyi2009generalized}) are known to coincide with their counterpart presented above.
Numerous studies have been done to further develop these approaches (see e.g.~\cite{dupuis2014decoupling,datta2013smooth,matthews2014finite,datta2011apex,qi2018applications,datta2016second,anshu2018building,anshu2019near,tomamichel2016quantum}).
However, the one-shot capacity theorem that reduces in the asymptotic limit to the result by Hsieh and Wilde \cite{hsieh2010entanglement} has not been obtained so far.

%and the private classical capacity is analyzed in \cite{salek2018one,renes2011noisy,radhakrishnan2017one,wilde2017position,}.

In this paper, we derive a one-shot generalization of the three-dimensional rate region obtained in \cite{hsieh2010entanglement}. 
Namely, we consider a task in which classical and quantum messages are transmitted via a noisy quantum channel with the assistance of a limited amount of shared entanglement, all in the one-shot scenario. 
The main result is that we derive inner and outer bonds for a one-shot rate region, which are represented in terms of the smooth conditional entropy of the channel.
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
In the asymptotic limit of infinitely many uses of the channel, the direct and converse bounds match and coincide with the achievable rate region obtained in \cite{hsieh2010entanglement}.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases, such as the Holevo-Schumacher-Westmoreland theorem \cite{holevo98,schumacher97} and the Lloyd-Shor-Devetak theorem \cite{lloyd1997capacity,shor2002quantum,devetak2005private}, are obtained from their result as corollaries.
Hence, our one-shot result result also recovers the capacity theorems in the asymptotic limit in those special cases.
Besides, the direct and converse bounds for various communication tasks in the one-shot scenario readily follow from our result.
It should be noted, however, that in special cases our result is not necessarily as strong as those in the previous literature.
To compare our result in detail with those in the previous literature is left as a future work.


The proof is based on the notion of {\it randomized partial decoupling} \cite{wakakuwa2021one}, which is a generalization of decoupling \cite{berry05,horo07,ADHW2009,patr08,DBWR2010,majenz2017catalytic}.
Here, we consider a scenario in which a bipartite quantum state on system $AR$ is subject to a unitary operation on $A$, followed by the action of a linear completely-positive (CP) map. Unlike the usual setting of decoupling, we assume that
the subsystem is decomposed into a direct-sum form, and 
the unitary is chosen at random from the set of unitaries that are block-diagonal under the decomposition. 
In \cite{wakakuwa2021one}, we proved the {\it randomized partial decoupling theorem}, which shows that the distance between the final state and the averaged one is bounded in terms of smooth conditional entropies of the initial state and the channel.
The previous results of the one-shot decoupling theorem \cite{DBWR2010} and the dequantization theorem \cite{dupuis2014decoupling}
are obtained from this result as corollaries (see Section III D in \cite{wakakuwa2021one} for the details).
In this paper, we apply the randomized partial decoupling theorem to the channel coding scenario to prove the one-shot capacity theorems.



This paper is organized as follows. 
In \rSec{prelimi}, we introduce notations and definitions that will be used throughout this paper. 
In \rSec{mainresults}, we present formulations of the problem and the main results. 
In \rSec{RPD}, we summarize the statement of the randomized partial decoupling theorem.
The proofs of the main theorems are provided in Section \rsec{direct} and \rsec{converse}.
In \rSec{iid}, we apply the one-shot results to the asymptotic limit of infinitely many uses of the channel, and obtain a three-dimensional achievable rate region region that is equivalent to the one obtained by Hsieh and Wilde.
A proof of the asymptotic result is provided in \rSec{PRFasymptotic}.
In \rSec{comparison}, we apply our results to special cases where one or only one or two resources are considered, and compare the results to those in the previous literature.
Conclusions are presented in \rSec{cncl}.




==> introduction_6.tex <==




One of the major goals of quantum communication theory is to investigate the ultimate capacities of a noisy quantum channel for transmitting classical and quantum information (see, e.g., \cite{wildetext,nielsentext}).
In an asymptotic limit of infinitely many uses of a memoryless channel, 
the classical capacity of a noisy quantum channel was obtained by Holevo \cite{holevo98}, Schumacher and Westmoreland  \cite{schumacher97};
the quantum capacity by Lloyd \cite{lloyd1997capacity}, Shor \cite{shor2002quantum} and Devetak \cite{devetak2005private};
the entanglement-assisted classical capacity by Bennet {\it et al.} \cite{bennett1999entanglement,bennett2002entanglement} and Shor \cite{shor2004classical};
the entanglement-assisted quantum capacity by Devetak {\it et al.} \cite{devetak2004family,deve08};
and the capacity of a quantum channel for simultaneously transmitting classical and quantum messages was obtained by Devetak and Shor \cite{devetak2005capacity}.
One of the most general results in this direction is provided by Hsieh and Wilde \cite{hsieh2010entanglement}, which obtained the triple trade-off among the resources of classical communication, and quantum communication and entanglement in quantum channel coding.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases mentioned above are obtained from their result as corollaries.


A modern approach addresses the same communication tasks under the assumption that the channel is used only once, which is referred to as the {\it one-shot} regime.
Along this line, the classical capacity of a noisy quantum channel was first investigated by Mosonyi {\it et al.} \cite{mosonyi2009generalized} and was developed by Renes {\it et al.} \cite{renes2011noisy} and Wang {\it et al.} \cite{wang2012one};
the quantum capacity was obtained by Buscemi {\it et al.}\cite{buscemi2010quantum};
the entanglement-assisted classical and quantum capacities by Datta {\it et al.} \cite{datta2012one};
and the capacity region for simultaneously transmitting classical and quantum information was obtained by Salek {\it et al.} \cite{salek2019one}.
In the asymptotic limit of infinitely many uses of a memoryless channel, all these results (except \cite{mosonyi2009generalized}) are known to coincide with their counterpart presented above.
Numerous studies have been done to further develop these approaches (see e.g.~\cite{dupuis2014decoupling,datta2011apex,datta2013smooth,matthews2014finite,datta2016second,tomamichel2016quantum,qi2018applications,anshu2018building,anshu2019near}).
However, the one-shot capacity theorem that reduces in the asymptotic limit to the result by Hsieh and Wilde \cite{hsieh2010entanglement} has not been obtained so far.

%and the private classical capacity is analyzed in \cite{salek2018one,renes2011noisy,radhakrishnan2017one,wilde2017position,}.

In this paper, we derive a one-shot generalization of the three-dimensional rate region obtained in \cite{hsieh2010entanglement}. 
Namely, we consider a task in which classical and quantum messages are transmitted via a noisy quantum channel with the assistance of a limited amount of shared entanglement, all in the one-shot scenario. 
The main result is that we derive inner and outer bonds for a one-shot rate region, which are represented in terms of the smooth conditional entropy of the channel.
To our knowledge, this is the first time that trade-off relations that applies simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
In the asymptotic limit of infinitely many uses of the channel, the direct and converse bounds match and coincide with the achievable rate region obtained in \cite{hsieh2010entanglement}.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases, such as the Holevo-Schumacher-Westmoreland theorem \cite{holevo98,schumacher97} and the Lloyd-Shor-Devetak theorem \cite{lloyd1997capacity,shor2002quantum,devetak2005private}, are obtained from their result as corollaries.
Hence, our one-shot result result also recovers the capacity theorems in the asymptotic limit in those special cases.
Besides, the direct and converse bounds for various communication tasks in the one-shot scenario readily follow from our result.
It should be noted, however, that in special cases our result is not necessarily as strong as those in the previous literature.
To compare our result in detail with those in the previous literature is left as a future work.


The proof is based on the notion of {\it randomized partial decoupling} \cite{wakakuwa2021one}, which is a generalization of decoupling \cite{berry05,horo07,ADHW2009,patr08,DBWR2010,majenz2017catalytic}.
Here, we consider a scenario in which a bipartite quantum state on system $AR$ is subject to a unitary operation on $A$, followed by the action of a linear completely-positive (CP) map. Unlike the usual setting of decoupling, we assume that
the subsystem is decomposed into a direct-sum form, and 
the unitary is chosen at random from the set of unitaries that are block-diagonal under the decomposition. 
In \cite{wakakuwa2021one}, we proved the {\it randomized partial decoupling theorem}, which shows that the distance between the final state and the averaged one is bounded in terms of smooth conditional entropies of the initial state and the channel.
The previous results of the one-shot decoupling theorem \cite{DBWR2010} and the dequantization theorem \cite{dupuis2014decoupling}
are obtained from this result as corollaries, up to changes of the smoothing parameters and the error parameters (see Section III D in \cite{wakakuwa2021one} for the details).
In this paper, we apply the randomized partial decoupling theorem to the channel coding scenario to prove the one-shot capacity theorems.



This paper is organized as follows. 
In \rSec{prelimi}, we introduce notations and definitions that will be used throughout this paper. 
In \rSec{mainresults}, we present formulations of the problem and the main results. 
In \rSec{RPD}, we summarize the statement of the randomized partial decoupling theorem.
The proofs of the main theorems are provided in Section \rsec{direct} and \rsec{converse}.
In \rSec{iid}, we apply the one-shot results to the asymptotic limit of infinitely many uses of the channel, and obtain a three-dimensional achievable rate region region that is equivalent to the one obtained by Hsieh and Wilde.
A proof of the asymptotic result is provided in \rSec{PRFasymptotic}.
In \rSec{comparison}, we apply our results to special cases where one or only one or two resources are considered, and compare the results to those in the previous literature.
Conclusions are presented in \rSec{cncl}.




==> introduction_7.tex <==




One of the major goals of quantum communication theory is to investigate the ultimate capacities of a noisy quantum channel for transmitting classical and quantum information (see, e.g., \cite{wildetext,nielsentext}).
In an asymptotic limit of infinitely many uses of a memoryless channel, 
the classical capacity of a noisy quantum channel was obtained by Holevo \cite{holevo98}, Schumacher and Westmoreland \cite{schumacher97};
the quantum capacity by Lloyd \cite{lloyd1997capacity}, Shor \cite{shor2002quantum} and Devetak \cite{devetak2005private};
the entanglement-assisted classical capacity by Bennet {\it et al.} \cite{bennett1999entanglement,bennett2002entanglement} and Shor \cite{shor2004classical};
the entanglement-assisted quantum capacity by Devetak {\it et al.} \cite{devetak2004family,deve08};
and the capacity of a quantum channel for simultaneously transmitting classical and quantum messages was obtained by Devetak and Shor \cite{devetak2005capacity}.
One of the most general results in this direction was shown by Hsieh and Wilde \cite{hsieh2010entanglement}, which provides a complete characterization of the triple trade-off among the resources of classical communication, quantum communication, and entanglement in quantum channel coding.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases mentioned above are obtained from their result as corollaries.


A modern approach addresses the same communication tasks under the assumption that the channel is used only once, which is referred to as the {\it one-shot} regime.
Along this line, the classical capacity of a noisy quantum channel was first investigated by Mosonyi {\it et al.} \cite{mosonyi2009generalized} and was developed by Renes {\it et al.} \cite{renes2011noisy} and Wang {\it et al.} \cite{wang2012one};
the quantum capacity was obtained by Buscemi {\it et al.}\cite{buscemi2010quantum};
the entanglement-assisted classical and quantum capacities by Datta {\it et al.} \cite{datta2012one};
and the capacity region for simultaneously transmitting classical and quantum information was obtained by Salek {\it et al.} \cite{salek2019one}.
In the asymptotic limit of infinitely many uses of a memoryless channel, all these results (except \cite{mosonyi2009generalized}) are known to coincide with the preexisting results presented above.
Numerous studies have been done to develop these approaches further (see e.g.~\cite{dupuis2014decoupling,datta2011apex,datta2013smooth,matthews2014finite,datta2016second,tomamichel2016quantum,qi2018applications,anshu2018building,anshu2019near}).
However, the one-shot capacity theorem that reduces in the asymptotic limit to the result by Hsieh and Wilde \cite{hsieh2010entanglement} has not been obtained so far.



In this paper, we derive a one-shot generalization of the three-dimensional rate region obtained in \cite{hsieh2010entanglement}. 
Namely, we consider a task in which classical and quantum messages are transmitted via a noisy quantum channel with the assistance of a limited amount of shared entanglement, all in the one-shot scenario. 
The main result is that we derive inner and outer bonds for the one-shot rate region, which are represented in terms of the smooth conditional entropy of the channel.
To our knowledge, this is the first time that trade-off relations that apply simultaneously to all the three resources of classical communication, quantum communication, and shared entanglement has been obtained in the one-shot channel coding scenario.
In the asymptotic limit of infinitely many uses of the channel, the direct and converse bounds match and coincide with the achievable rate region obtained in \cite{hsieh2010entanglement}.
As proved in \cite{hsieh2010entanglement}, the capacity theorems in the special cases, such as the Holevo-Schumacher-Westmoreland theorem \cite{holevo98,schumacher97} and the Lloyd-Shor-Devetak theorem \cite{lloyd1997capacity,shor2002quantum,devetak2005private}, are obtained from their result as corollaries.
Hence, our one-shot result also recovers the capacity theorems in the asymptotic limit in those special cases.
Besides, the direct and converse bounds for various communication tasks in the one-shot scenario readily follow from our result.
It should be noted, however, that in special cases, our result is not necessarily as strong as those in the previous literature.
To compare our results in detail with those in the previous literature is left as a future work.


The proof is based on the notion of {\it randomized partial decoupling} \cite{wakakuwa2021one}, which is a generalization of decoupling \cite{berry05,horo07,ADHW2009,patr08,DBWR2010,majenz2017catalytic}.
Here, we consider a scenario in which a bipartite quantum state on system $AR$ is subject to a unitary operation on $A$, followed by the action of a linear completely positive (CP) map. Unlike the usual setting of decoupling, we assume that
the subsystem is decomposed into a direct-sum form, and 
the unitary is chosen at random from the set of unitaries that are block-diagonal under the decomposition. 
In \cite{wakakuwa2021one}, we proved the {\it randomized partial decoupling theorem}, which shows that the distance between the final state and the averaged one is bounded in terms of smooth conditional entropies of the initial state and the channel.
The previous results of the one-shot decoupling theorem \cite{DBWR2010} and the dequantization theorem \cite{dupuis2014decoupling}
are obtained from this result as corollaries, up to changes in the smoothing and error parameters (see Section III D in \cite{wakakuwa2021one} for the details).
The current paper applies the randomized partial decoupling theorem to the channel coding scenario for proving the one-shot capacity theorems.



This paper is organized as follows. 
In \rSec{prelimi}, we introduce notations and definitions that will be used throughout this paper. 
In \rSec{mainresults}, we present formulations of the problem and state the main results. 
In \rSec{RPD}, we summarize the statement of the randomized partial decoupling theorem.
The proofs of the main theorems are provided in Section \rsec{direct} and \rsec{converse}.
In \rSec{iid}, we apply the one-shot results to the asymptotic scenario of infinitely many uses of the channel and obtain a three-dimensional achievable rate region that is equivalent to the one obtained by Hsieh and Wilde.
Proof of the asymptotic result is provided in \rSec{PRFasymptotic}.
In \rSec{comparison}, we apply our results to special cases where one or two of the three resources are assumed to be zero and compare the results to those in the previous literature.
Conclusions are presented in \rSec{cncl}.



